Minimal Perspective Autocalibration

We introduce a new family of minimal problems for reconstruction from multiple views. Our primary focus is a novel approach to autocalibration, a long-standing problem in computer vision. Traditional approaches to this problem, such as those based on Kruppa's equations or the modulus constraint, rely explicitly on the knowledge of multiple fundamental matrices or a projective reconstruction. In contrast, we consider a novel formulation involving constraints on image points, the unknown depths of 3D points, and a partially specified calibration matrix $K$. For $2$ and $3$ views, we present a comprehensive taxonomy of minimal autocalibration problems obtained by relaxing some of these constraints. These problems are organized into classes according to the number of views and any assumed prior knowledge of $K$. Within each class, we determine problems with the fewest -- or a relatively small number of -- solutions. From this zoo of problems, we devise three practical solvers. Experiments with synthetic and real data and interfacing our solvers with COLMAP demonstrate that we achieve superior accuracy compared to state-of-the-art calibration methods. The code is available at https://github.com/andreadalcin/MinimalPerspectiveAutocalibration

==> commands.tex <==

\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\newcommand{\TP}[1]{\textcolor{brown}{TP: #1}}
\newcommand{\tim}[1]{\textcolor{red}{TD: #1}}
\newcommand{\AP}[1]{\textcolor{blue}{AP: #1}}
\newcommand{\lm}[1]{\textcolor{teal}{LM: #1}}

\newcommand{\CC}{{\mathbb C}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\TT}[1]{{$\mathtt{#1}$}}
\newcommand{\RED}{\textcolor{red}{R}}
\newcommand{\BLACK}{B}
\newcommand{\BLUE}{\textcolor{blue}{B}}
\newcommand{\GREEN}{\textcolor{green}{G}}
\newcommand{\WHITE}{W}
\definecolor{mypurp}{RGB}{128,0,128}
\newcommand{\colset}{\{ \BLUE, \RED, \GREEN, \WHITE \}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newcommand{\VV}{\mathbb{V}}

\newcommand{\arr}[2]{\begin{array}{#1} #2\end{array}}
\newcommand{\mat}[2]{\left(\!\!\arr{#1}{#2}\!\!\right)}
\renewcommand{\vec}{{}}
\newcommand{\M}{{}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\pp}{\mathbf{p}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\LL}{\mathcal{L}}

==> min_problem_and_relaxation_bkp.tex <==
\textbf{Minimal problems and minimal relaxations.}

Many estimation problems in vision are special cases of the following general problem. 
Consider an algebraic variety $X$, whose points consist of problem-solution pairs $(\pp,\xx) \in \CC^m \times \CC^n$ satisfying some set of equations depending polynomially on $\pp $ and $\xx .$
We assume that the variety $X$ is \emph{irreducible} (cf.~\cite[\S 5]{Cox-IVA-2015}.)
Our task is to compute a solution $\xx \in \CC^n$ for some problem instance $\pp\in \CC^m,$ meaning $(\pp , \xx) \in X.$ 
If we consider the projection map from $X$ into the space of problem instances,
\begin{align}
\pi : X &\to \CC^m, \nonumber \\
(\pp,\xx) &\mapsto \pp, \label{eq:pi-map}
\end{align}
then the set of solutions of a particular problem instance $\pp \in \CC^m$ may be identified with the fiber $\pi^{-1} (\pp)$.
Following~\cite{DBLP:conf/iccv/DuffKLP19}, we say that $\pi $ defines \emph{minimal problem} if
\begin{enumerate}
    \item \label{minimal-condition-1} The problem is \emph{balanced}---that is, $\dim X = m.$
    \item \label{minimal-condition-2} Almost every problem instance in $\CC^m$ has a solution---equivalently, the image of the map $\pi $ is dense in $\CC^m.$
\end{enumerate}
In practice, we check that a problem is minimal using some system of equations $\bg (\pp , \xx) = 0$ defining $X$ locally, via the following \emph{rank conditions} at a point $(\pp_0, \xx_0) \in X$: 
\begin{align}
    \operatorname{rank} \left( \frac{\partial \bg}{\partial \pp } \mid \frac{\partial \bg}{\partial \xx} \right)\Big\vert_{(\pp_0, \xx_0)} &= n, \label{eq:rank-condition-balanced}\\
    \operatorname{rank} \left( \frac{\partial \bg}{\partial \xx} \right)\Big\vert_{(\pp_0, \xx_0)} &= n .\label{eq:rank-condition-zero-dim}
\end{align}

In our formulation of autocalibration, we may generally take as $\pp = (x_{ip})_{i \in [M], p\in [N]}$ the image points.
The unknowns $\xx$ may either be some subset of the unknowns $(R_i), (X_p), (\lambda_{ip})$, 
suitably normalized according to the ambiguity~\eqref{eq:ambiguity}, or the parameters defining $\omega $ in~\eqref{eq:omega}.
In all such cases, the variety $X$ is the image of the graph of a suitably-defined \emph{joint camera map} (cf.~\cite[\S 4]{DBLP:conf/iccv/DuffKLP19}), and therefore $X$ is irreducible.

Some of the cases appearing in~\Cref{tab:Minimal-Autocalibration-Substitution-Tab} are already minimal problems.
These are precisely the rows where $\# G = 1$, in which case both sides of~\eqref{eq:L-lower-bound} are equal.
In general, we have $\dim X = 3N + 6M -2 - L,$ and $m= 2MN.$

When the inequality~\eqref{eq:L-lower-bound} is strict, we expect the autocalibration problem~\eqref{eq:zx=K[R|-RC][X;;]} to be \emph{overconstrained} in the sense that a generic problem in $\CC^m$ does not have a solution.

To deal with overconstrained problems, consider a system $\bg$ consisting of $n$ polynomial or rational functions vanishing on $X$---that is, $X \subset \VV (\bg )$ where 
\begin{equation}\label{eq:Vg}
\VV (\bg ) = 
\overline{\{ (\pp , \xx) \in \CC^{m+n} \mid \bg(\xx ; \pp) \text{ is defined and equals } 0 \}}
\end{equation}
($\overline{\bullet }$ denotes the Zariski closure~\cite[\S 4.4]{CLO}.)
If the rank conditions~\eqref{eq:rank-condition-balanced}--\eqref{eq:rank-condition-zero-dim} hold at a generic point $(\pp_0, \xx_0)\in X,$ we say that $\bg$ determines a \emph{minimal relaxation} of $\pi .$
With this definition, we note that the variety $\overline{\VV (\bg)}$ that ``relaxes" the irreducible $X$ may be reducible.
Nevertheless, it follows from the rank conditions~\eqref{eq:rank-condition-balanced}--\eqref{eq:rank-condition-zero-dim} that a generic point on $X$ is a smooth point of $\overline{\VV (\bg)}$, and hence lies on a unique irreducible component $X_{\bg}$ of $\overline{\VV (\bg)}$.
From this fact, we may conclude that the associated projection $\pi_{\bg} : X_{\bg} \to \CC^m$ defines a minimal problem in the sense given above.
We refer to the supplementary material for a detailed discussion, illustrating various technicalities in our definition of a minimal relaxation.

In general, an overconstrained problem can have different minimal relaxations.
In the next section, we obtain a combinatorial classification of all minimal relaxations obtained from subsets of the depth constraints~\eqref{eq:depth-equation-2}.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{comment}
\usepackage[utf8]{inputenc}
\usepackage{xcolor}
\usepackage{arydshln}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{listings}
\usepackage{pbox}
\usepackage{enumitem}
\usepackage{diagbox}
\usepackage{xspace}

\newcommand{\hide}[1]{}
\newcommand{\RANSAC}{\textsc{RanSaC}}
\usepackage{stfloats}

\newif\ifsupplementary

==> tables/table-L.tex <==
\medskip
\noindent
\textbf{Minimum number of points.} 
\begin{table}[]
    \centering
    \begin{tabular}{c|ccccccc}
        $M\, $ \textbackslash $\, L$ &  0 & 1 & 2 & 3 & 4 & 5  \\
        \hline  
        2 & $\infty $ & $\infty $ & $\infty $ & 7 & 6 & 5\\
        3 & 6 & 5 & 5 & 5 & 4 & 4
    \end{tabular}
    \caption{Minimum number of points needed to autocalibrate with $L$ linear constraints on $K$ from image data in $M\in \{ 2, 3 \} $ views.}
    \label{tab:minimum-L-M}
\end{table}

==> tables/table-autocalibration-full.tex <==
\begin{table*}[h]
    \centering
    {\tiny
    \begin{tabular}{|ccc|c|cccccccccc|cc|l|} \hline
         Intrinsics &$M$&$N$&$L$&  1      &  2   &  3   & 4 & 5 & 6 & 7 & 8 & 9 & 10 & T & $\# G$ & Literature \\ \hline
         \TT{fguvs} & 2 & - & 0 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\ 
         \TT{fguvs} & 3 & 6 & 0 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 5852925 & 1827 &   \\ \hline
         \TT{fguv0} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\ 
         \TT{fguv0} & 3 & 5 & 1 &2313    & 2313 & 2313 &   &   &   &   &   &   &    & 190 & 3 &   \\ \hline
         \TT{fgu0s} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\ 
         \TT{fgu0s} & 3 & 5 & 1 &2058    & 2058 & 2058 &   &   &   &   &   &   &    & 190 & 3 &   \\ \hline
         \TT{fgu00} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\ 
         \TT{fgu00} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 1140 & 8 & \\ \hline
         \TT{fg0vs} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\ 
         \TT{fg0vs} & 3 & 5 & 1 &2058    & 2058 & 2058 &   &   &   &   &   &   &    & 190 & 3 & \\ \hline
         \TT{fg0v0} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &  \\
         \TT{fg0v0} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 1140 & 8 & \\ \hline
         \TT{fg00s} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &  \\
         \TT{fg00s} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 1140 & 8 & \\ \hline
         \TT{fg000} & 2 & 7 & 3 &18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{fg000} & 3 & 5 & 3 &3884 & 3884 & 3884 & 3884 & 16356 & 16948 & 17364 & 17624 & 17624 & 17624 & 4845 & 35 & \\ \hline
         \TT{f1uvs} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{f1uvs} & 3 & 5 & 1 &4111 & 4111 & 4111 &   &   &   &   &   &   &    & 190 & 3 &   \\ \hline
         \TT{f1uv0} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{f1uv0} & 3 & 5 & 2 &29044	& 29044 & 29044 & 29044 & 29044 & 100816 & 100816 & 100816 & & & 1140 & 8 & \\ \hline
         \TT{f1u0s} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{f1u0s} & 3 & 5 & 2 &14760 & 14760 & 14760	& 14760 & 14760 & 53066 & 53066 & 53066 & & & 1140 & 8 & \\ \hline
         \TT{f1u00} & 2 & 7 & 3 &18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f1u00} & 3 & 5 & 3 &4400 & 4400 & 4400 & 4400 & 19072 & 20350 & 20480 & 20480 & 20480 & 23132 & 4845 & 35 & \\ \hline
         \TT{f10vs} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{f10vs} & 3 & 5 & 2 &24332	& 24332	& 24332	& 24332	& 24332 & 86530 & 86530 & 86530 & & & 1140 & 8 & \\ \hline
         \TT{f10v0} & 2 & 7 & 3 & 36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f10v0} & 3 & 5 & 3 &7764 & 7764 & 7764 & 7764 & 32679 & 33862 & 34680 & 35230 & 35230 & 35230 & 4845 & 35 & \\ \hline
         \TT{f100s} & 2 & 7 & 3 & 18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f100s} & 3 & 5 & 3 &4392 & 4392 & 4392 & 4392 & 19064 & 19846 & 20341 & 20480 & 20480 & 20480 & 4845 & 35 & \\ \hline
         \TT{f1000} & 2 & 6 & 4 &30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f1000} & 3 & 4 & 4 & 668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{1guvs} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{1guvs} & 3 & 5 & 1 &4360 & 4360 & 4360 &   &   &   &   &   &   &    & 190 & 3 &   \\ \hline
         \TT{1guv0} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{1guv0} & 3 & 5 & 2 &29046 & 29046 & 29046 & 29046 & 29046 & 100808 & 100808	& 100808 & & & 1140 & 8 &   \\ \hline
         \TT{1gu0s} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{1gu0s} & 3 & 5 & 2 &29024	& 29024	& 29024	& 29024	& 29024 & 100718 & 100718 & 100718 & & & 1140 & 8 & \\ \hline
         \TT{1gu00} & 2 & 7 & 3 & 36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ 
         \TT{1gu00} & 3 & 5 & 3 &7760 & 7760 & 7760 & 7760 & 33742 & 34542 & 35238 & 35238 & 35238 & 39362 & 4845 & 35 & \\ \hline
         \TT{1g0vs} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{1g0vs} & 3 & 5 & 2 &29012 & 29012 & 29012 & 29012 & 29012 & 100776 & 100776 & 100776 & & & 1140 & 8 & \\ \hline
         \TT{1g0v0} & 2 & 7 & 3 &18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g0v0} & 3 & 5 & 3 &4400 & 4400 & 4400 & 4400 & 19072 & 19856 & 20349 & 20480 & 20480 & 20480 & 4845 & 35 & \\ \hline
         \TT{1g00s} & 2 & 7 & 3 &24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g00s} & 3 & 5 & 3 &4480 & 4480 & 4480 & 4480 & 18807 & 19356 & 19769 & 20024 & 20024 & 20024 & 4845 & 35 & \\ \hline
         \TT{1g000} & 2 & 6 & 4 &30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g000} & 3 & 4 & 4 &668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{11uvs} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{11uvs} & 3 & 5 & 2 &57912 & 57912	& 57912 & 57912 & 57912 & 201264 & 201264	& 201264 & & & 1140 & 8 & \\ \hline
         \TT{11uv0} & 2 & 7 & 3 &48 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11uv0} & 3 & 5 & 3 &8940 & 8940 & 8940 & 8940 & 37602 & 38693 & 39511 & 40028 & 40028 & 40028 & 4845 & 35 & \\ \hline
         \TT{11u0s} & 2 & 7 & 3 &36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11u0s} & 3 & 5 & 3 &8786 & 8786 & 8786 & 8785 & 37996	& 39494	& 40447 & 40916 & 40916	& 40916 & 4845 & 35 &  \\ \hline
         \TT{11u00} & 2 & 6 & 4 & 60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11u00} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{110vs} & 2 & 7 & 3 &72 &      &      &   &   &   &   &   &   &    &  1 & 1 &   \\
         \TT{110vs} & 3 & 5 & 3 &16390 & 16390 & 16390 & 16390 & 70397 & 73100 & 75029 & 76046 & 76046 & 76046 & 4845 & 35 &   \\ \hline
         \TT{110v0} & 2 & 6 & 4 &60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{110v0} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{1100s} & 2 & 6 & 4 &60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1100s} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{11000} & 2 & 5 & 5 &20      &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11000} & 3 & 4 & 5 &640       &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{ffuvs} & 2 & - & 1 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{ffuvs} & 3 & 5 & 1 & 4617 & 4617 & 4617 &   &   &   &   &   &   &    & 190 & 3 &   \\ \hline
         \TT{ffuv0} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{ffuv0} & 3 & 5 & 2 &16188 & 16188 & 16188 & 16188 & 16188 & 55174 & 55174 & 55174 &   &    & 1140 & 8 &   \\ \hline
         \TT{ffu0s} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{ffu0s} & 3 & 5 & 2 &29028 & 29028 & 29028 & 29028 & 29028 & 100758 & 100758 & 100758 &   &    & 1140 & 8 &   \\ \hline
         \TT{ffu00} & 2 & 7 & 3 &24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ffu00} & 3 & 5 & 3 &4484 & 4484 & 4484 & 4484 & 18819 & 19761 & 20024 & 20024 & 20024 & 22254 & 4845 & 35 & \\ \hline
         \TT{ff0vs} & 2 & - & 2 &$\infty$ &      &      &   &   &   &   &   &   &    & 0 & 0 &   \\
         \TT{ff0vs} & 3 & 5 & 2 &38700 & 38700 & 38700 & 38700 & 38700 & 134352	& 134352 & 134352 &   &    & 1140 & 8 &   \\ \hline
         \TT{ff0v0} & 2 & 7 & 3 &24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff0v0} & 3 & 5 & 3 &4484 & 4484 & 4484	& 4484 & 18820 & 19359 & 19776 & 20024 & 20024 & 20024 & 4845 & 35 &  \\ \hline
         \TT{ff00s} & 2 & 7 & 3 &36 & & &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff00s} & 3 & 5 & 3 &7756 & 7756 & 7756 & 7756 & 32695 & 33869 & 34702 & 35238 & 35238 & 35236 & 4845 & 35 & \\ \hline
         \TT{ff000} & 2 & 6 & 4 & 30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff000} & 3 & 4 & 4 & 668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
    \end{tabular}
    }
\caption{Specification of 80 interesting minimal problems in $N = 2$ and $M = 3$ cameras. For each triplet $(\mathtt{fguvs},M,N)$ describing a minimal problem, the number of possible sets of constraints $\#G$ is reported. We also report the count of solutions in $\mathbb{C}$ for up to ten four-tuples $(\mathtt{fguvs},M,N,G)$. The solution counts refer to unknowns appearing the parametrization by $\omega $ as in equations~\eqref{eq:omega}--\eqref{eq:depth-equation-2}.}
% \label{tab:Minimal-Autocalibration-Substitution-Tab}
\end{table*}

==> tables/table-autocalibration-summary.tex <==
% \renewcommand{\arraystretch}{0.975}
\begin{table*}[h]
    \centering
    {\tiny
    \vspace{-2em}
    \begin{tabular}{|c|c|c|c|cccccccccc|c|c|l|} 
         \hline
         Prior on $K$ & $M$ & $N$ & $L$ & \multicolumn{10}{c|}{Solution count in $\mathbb{C}$ for the first 10 equivalence classes} & $\# \text{balanced} $ & $\# \bg$ & Literature \\ \hline
         \TT{fguvs} & 3 & 6 & 0 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 2985 & 4149855 & 3313 & \\ \hline 
         \TT{fguv0} & 3 & 5 & 1 &2313    & 2313 & 2313 &   &   &   &   &   &   &    & 100 & 3 &   \\ \hline 
         \TT{fgu0s} & 3 & 5 & 1 &2058    & 2058 & 2058 &   &   &   &   &   &   &    & 100 & 3 &   \\ \hline 
         \TT{fgu00} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 900 & 8 & \\ \hline 
         \TT{fg0vs} & 3 & 5 & 1 & 2058 & 2058 & 2058 &   &   &   &   &   &   &    & 100 & 3 & \\ \hline 
         \TT{fg0v0} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 900 & 8 & \\ \hline 
         \TT{fg00s} & 3 & 5 & 2 &9686 & 9686 & 9686 & 9686 & 9686 & 33606 & 33606 & 33606 & & & 900 & 8 & \\ \hline 
         \TT{fg000} & 2 & 7 & 3 & 18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{fg000} & 3 & 5 & 3 &3884 & 3884 & 3884 & 3884 & 16356 & 16948 & 17364 & 17624 & 17624 & 17624 & 4425 & 37 & \\ \hline
         \TT{f1uvs} & 3 & 5 & 1 &4111 & 4111 & 4111 &   &   &   &   &   &   &    & 100 & 3 &   \\ \hline 
         \TT{f1uv0} & 3 & 5 & 2 & 29044	& 29044 & 29044 & 29044 & 29044 & 100816 & 100816 & 100816 & & & 900 & 8 & \\ \hline
         \TT{f1u0s} & 3 & 5 & 2 &14760 & 14760 & 14760	& 14760 & 14760 & 53066 & 53066 & 53066 & & & 900 & 8 & \\ \hline 
         \TT{f1u00} & 2 & 7 & 3 & 18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ 
         \TT{f1u00} & 3 & 5 & 3 & 4400 & 4400 & 4400 & 4400 & 19072 & 20350 & 20480 & 20480 & 20480 & 23132 & 4425 & 37 & \\ \hline
         \TT{f10vs} & 3 & 5 & 2 &24332	& 24332	& 24332	& 24332	& 24332 & 86530 & 86530 & 86530 & & & 900 & 8 & \\ \hline 
         \TT{f10v0} & 2 & 7 & 3 & 36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f10v0} & 3 & 5 & 3 &7764 & 7764 & 7764 & 7764 & 32679 & 33862 & 34680 & 35230 & 35230 & 35230 & 4425 & 37 & \\ \hline
         \TT{f100s} & 2 & 7 & 3 & 18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f100s} & 3 & 5 & 3 &4392 & 4392 & 4392 & 4392 & 19064 & 19846 & 20341 & 20480 & 20480 & 20480 & 4425 & 37 & \\ \hline
         \TT{f1000} & 2 & 6 & 4 & 30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{f1000} & 3 & 4 & 4 & 668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{1guvs} & 3 & 5 & 1 &4360 & 4360 & 4360 &   &   &   &   &   &   &    & 100 & 3 &   \\ \hline 
         \TT{1guv0} & 3 & 5 & 2 &29046 & 29046 & 29046 & 29046 & 29046 & 100808 & 100808	& 100808 & & & 900 & 8 &   \\ \hline 
         \TT{1gu0s} & 3 & 5 & 2 &29024	& 29024	& 29024	& 29024	& 29024 & 100718 & 100718 & 100718 & & & 900 & 8 & \\ \hline 
         \TT{1gu00} & 2 & 7 & 3 & 36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1gu00} & 3 & 5 & 3 &7760 & 7760 & 7760 & 7760 & 33742 & 34542 & 35238 & 35238 & 35238 & 39362 & 4425 & 37 & \\ \hline
         \TT{1g0vs} & 3 & 5 & 2 &29012 & 29012 & 29012 & 29012 & 29012 & 100776 & 100776 & 100776 & & & 900 & 8 & \\ \hline 
         \TT{1g0v0} & 2 & 7 & 3 & 18 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g0v0} & 3 & 5 & 3 &4400 & 4400 & 4400 & 4400 & 19072 & 19856 & 20349 & 20480 & 20480 & 20480 & 4425 & 37 & \\ \hline
         \TT{1g00s} & 2 & 7 & 3 & 24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g00s} & 3 & 5 & 3 &4480 & 4480 & 4480 & 4480 & 18807 & 19356 & 19769 & 20024 & 20024 & 20024 & 4425 & 37 & \\ \hline
         \TT{1g000} & 2 & 6 & 4 &30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1g000} & 3 & 4 & 4 & 668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{11uvs} & 3 & 5 & 2 & 57912 & 57912	& 57912 & 57912 & 57912 & 201264 & 201264	& 201264 & & & 900 & 8 & \\ \hline 
         \TT{11uv0} & 2 & 7 & 3 &48 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11uv0} & 3 & 5 & 3 &8940 & 8940 & 8940 & 8940 & 37602 & 38693 & 39511 & 40028 & 40028 & 40028 & 4425 & 37 & \\ \hline
         \TT{11u0s} & 2 & 7 & 3 &36 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11u0s} & 3 & 5 & 3 &8786 & 8786 & 8786 & 8785 & 37996	& 39494	& 40447 & 40916 & 40916	& 40916 & 4425 & 37 &  \\ \hline
         \TT{11u00} & 2 & 6 & 4 & 60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11u00} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{110vs} & 2 & 7 & 3 &72 &      &      &   &   &   &   &   &   &    &  1 & 1 &   \\
         \TT{110vs} & 3 & 5 & 3 &16390 & 16390 & 16390 & 16390 & 70397 & 73100 & 75029 & 76046 & 76046 & 76046 & 4425 & 37 &   \\ \hline
         \TT{110v0} & 2 & 6 & 4 &60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{110v0} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{1100s} & 2 & 6 & 4 &60 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{1100s} & 3 & 4 & 4 &1336    &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{11000} & 2 & 5 & 5 &20      &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{11000} & 3 & 4 & 5 &640       &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
         \TT{ffuvs} & 3 & 5 & 1 & 4617 & 4617 & 4617 &   &   &   &   &   &   &    & 100 & 3 &   \\ \hline 
         \TT{ffuv0} & 3 & 5 & 2 &16188 & 16188 & 16188 & 16188 & 16188 & 55174 & 55174 & 55174 &   &    & 900 & 8 &   \\ \hline 
         \TT{ffu0s} & 3 & 5 & 2 &29028 & 29028 & 29028 & 29028 & 29028 & 100758 & 100758 & 100758 &   &    & 900 & 8 &   \\ \hline 
         \TT{ffu00} & 2 & 7 & 3 &24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ffu00} & 3 & 5 & 3 &4484 & 4484 & 4484 & 4484 & 18819 & 19761 & 20024 & 20024 & 20024 & 22254 & 4425 & 37 & \\ \hline
         \TT{ff0vs} & 3 & 5 & 2 &38700 & 38700 & 38700 & 38700 & 38700 & 134352	& 134352 & 134352 &   &    & 900 & 8 &   \\ \hline 
         \TT{ff0v0} & 2 & 7 & 3 &24 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff0v0} & 3 & 5 & 3 &4484 & 4484 & 4484	& 4484 & 18820 & 19359 & 19776 & 20024 & 20024 & 20024 & 4425 & 37 &  \\ \hline
         \TT{ff00s} & 2 & 7 & 3 &36 & & &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff00s} & 3 & 5 & 3 &7756 & 7756 & 7756 & 7756 & 32695 & 33869 & 34702 & 35238 & 35238 & 35236 & 4425 & 37 & \\ \hline
         \TT{ff000} & 2 & 6 & 4 &30 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\
         \TT{ff000} & 3 & 4 & 4 &668 &      &      &   &   &   &   &   &   &    & 1 & 1 &   \\ \hline
    \end{tabular}
    }
\caption{\textbf{Minimal Autocalibration.} Specification of 60 minimal problems in 2 and 3 views $M$. For each problem $(\mathtt{fguvs},M,N)$, we report: \emph{i}) $L$, number of linear constraints on $K$, \emph{ii}) $\# \text{balanced} $, all possible subsets of constraints \cref{eq:depth-equation-2} leading to a balanced problem, \emph{iii}) $\# \bg$, number of equivalence classes of constraints leading to a minimal problem, \emph{iv}) count of solutions in $\mathbb{C}$ for up to ten four-tuples $(\mathtt{fguvs},M,N, \bg)$ (in ascending order). The solution counts refer to unknowns appearing in the parameterization by $\omega $ as in Eqs.~\eqref{eq:omega}--\eqref{eq:depth-equation-2}.}
\label{tab:Minimal-Autocalibration-Substitution-Tab}
\end{table*}

==> tables/table-exp-colmap.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[tp]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccccccccc@{}}
\toprule
& \multicolumn{4}{c}{Fountain-P11}
& \multicolumn{4}{c}{Rathaus}
& \multicolumn{4}{c}{KITTI-Depth} \\
\cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13}
Variant &
  $\Delta fg \downarrow$ &
  $\Delta uv \downarrow$ &
  $Re$ &
  Points3D &
  $\Delta fg \downarrow$ &
  $\Delta uv \downarrow$ &
  $Re$ &
  Points3D &
  $\Delta fg \downarrow$ &
  $\Delta uv \downarrow$ &
  $Re$ &
  Points3D \\ \midrule
$\text{COLMAP}_\mathrm{guess}$ & 0.3350 & 0.0140 & 0.444 & 4848 & 0.0671 & 0.0812 & 0.624 & 847 & 0.6510 & 0.1360 & 0.810 & 210 \\
$\text{COLMAP}_\texttt{fguv0}$ & 0.0058 & 0.0297 & 0.241 & 5356 & 0.0237 & \textbf{0.0111} & 0.450 & 823 & \textbf{0.0720} & \textbf{0.0185} & 0.409 & 231 \\
$\text{COLMAP}_\mathrm{guess}$ + $K\text{-BA}$ & 0.0012 & 0.0013 & 0.212 & 5296 & 0.0185 & 0.0607 & 0.435 & 868 & 0.3480 & 0.5072 & 0.547 & 232 \\
$\text{COLMAP}_\texttt{fguv0}$ + $K\text{-BA}$ & \textbf{0.0011} & \textbf{0.0012} & 0.212 & 5367 & \textbf{0.0165} & 0.0307 & 0.432 & 823 & 0.0626 & 0.1773 & 0.404 & 236 \\ \midrule
$\text{COLMAP}_\mathrm{gt}$ + $K\text{-BA}$ & 0.0013 & 0.0011 & 0.210 & 5368 & 0.0069 & 0.0291 & 0.430 & 794 & 0.0401 & 0.0553 & 0.398 & 237 \\ 
\bottomrule
\end{tabular}
}
\caption{
Comparing errors and numbers of registered points for autocalibration strategies in COLMAP (\cref{sec:experiments-colmap}.)
%\textbf{Autocalibration in COLMAP.
} 
% Results obtained by COLMAP variants in real image sequences. In the top block, we compare the camera calibration attained by the standard COLMAP initialization method ($K_\mathrm{guess}$) with the results achieved by the \texttt{fguv0} solver. In the second block, we compare the results after running Bundle Adjustment, commencing from either the COLMAP-initialized parameters ($K_\mathrm{guess}$ + BA) or the parameters from \texttt{fguv0} ($K_\mathrm{guess}$ + BA). We include reference performance for COLMAP with ground truth intrinsics and Bundle Adjustment. \AP{Update notation.}}
\label{tab:experiments-colmap}
\end{table*}

==> tables/table-exp-real.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[t]
\centering
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule
 &
  \multicolumn{7}{c}{Fountain-P11} &
  \multicolumn{7}{c}{Herz-Jesu-P8} \\
  \cmidrule(l){2-8} \cmidrule(l){9-15}
Method &
  $\Delta fg$ &
  $\Delta uv$ &
  $\Delta s$ &
  $Re_\mathrm{gt}$ &
  $Re$ &
  $\epsilon_R$ &
  $\epsilon_C$ &
  $\Delta fg$ &
  $\Delta uv$ &
  $\Delta s$ &
  $Re_\mathrm{gt}$ &
  $Re$ &
  $\epsilon_R$ &
  $\epsilon_C$ \\ \midrule
  Kruppa-6 & 0.137 & 0.184 & 0.022 & 19.563 & 2.891 & 7.061 & 5.579 & 0.098 & 0.112 & 0.014 & 14.565 & 1.112 & 2.125 & 1.902 \\
  Kruppa-7 & 0.249 & 0.204 & 0.040 & 28.197 & - & - & - & 0.122 & 0.114 & 0.040 & 15.252 & - & - & - \\
  Kruppa-8 \cite{LuongF97} & 0.260 & 0.173 & 0.029 & 28.466 & - & - & - & 0.140 & 0.115 & 0.022 & 13.606 & - & - & - \\
  Kruppa BnB \cite{paudel2018sampling} & 0.127 & 0.058 & 0.014 & 9.231 & - & - & - & 0.078 & 0.096 & 0.018 & 21.023 & - & - & - \\
  Modulus BnB \cite{paudel2018sampling} & 0.162 & 0.071 & 0.016 & 10.540 & - & - & - & 0.097 & 0.102 & 0.019 & 22.641 & - & - & - \\
  \midrule
  \TT{ffuv0} & \textbf{0.017} & \textbf{0.029} & - & \textbf{4.435} & \textbf{0.449} & \textbf{0.623} & \textbf{0.664} & \textbf{0.017} & \textbf{0.044} & - & \textbf{8.082} & \textbf{0.672} & \textbf{0.664} & \textbf{0.656} \\
  \TT{fguv0} & 0.028 & 0.050 & - & 8.580 & 0.554 & 0.970 & 1.183 & 0.029 & 0.063 & - & 11.128 & 0.680 & 1.295 & 1.540 \\
  \TT{fguvs} & 0.035 & 0.064 & \textbf{0.008} & 9.769 & 1.075 & 1.274 & 1.428 & 0.041 & 0.058 & \textbf{0.013} & 11.348 & 0.989 & 1.085 & 1.139 \\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{Autocalibration Evaluation on Real Datasets.} 
Mean relative errors in the focal lengths $\Delta fg$, principal point $\Delta uv$, and skew $\Delta s$ are reported. Reprojection error is computed in two variations: \emph{i}) $Re_\mathrm{gt}$, using estimated $K$ and ground truth camera poses, \emph{ii}) $Re$, using estimated $K$ and estimated camera poses (when applicable). $\epsilon_R$ and $\epsilon_C$ are the angular errors in estimated camera rotations and translations, respectively. Lower values indicate better performance for all metrics.}
\label{tab:experiments-real}
\vspace{-0.5em}
\end{table*}

==> tables/table-small.tex <==
% \renewcommand{\arraystretch}{0.975}
\begin{table*}[ht]
    \centering
    {\tiny
    \vspace{-2.0em}
    \begin{tabular}{|c|c|c|c|cc|c|c||c|c|c|c|cc|c|c|} 
         \hline
         Prior on $K$ & $M$ & $N$ & $L$ & Min \# sol. in $\mathbb{C}$ & Max \# sol. in $\mathbb{C}$ & \# subsys. & $\# \bg$ & Prior on $K$ & $M$ & $N$ & $L$ & Min \# sol. in $\mathbb{C}$ & Max \# sol. in $\mathbb{C}$ & \# subsys. & $\# \bg$ \\ \hline
         \TT{fguvs} & 2 & - & 0 & $\infty$ & $\infty$ & 0 & 0 & \TT{1g0vs} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 \\ 
         \TT{fguvs} & 3 & 6 & 0 & 2985$^\ast $ & 1136202$^\ast$ & 5852925 & 3313 & \TT{1g0vs} & 3 & 5 & 2 & 29012 & 315653 & 1140 & 8 \\ \hline 
         \TT{fguv0} & 2 & - & 1 & $\infty$ & $\infty$ & 0 & 0 & \TT{1g0v0} & 2 & 7 & 3 & 18 & 18 & 1 & 1 \\ 
         \TT{fguv0} & 3 & 5 & 1 & 2313 & 2313 & 190 & 3 & \TT{1g0v0} & 3 & 5 & 3 & 4400 & 102784 & 4845 & 37 \\ \hline 
         \TT{fgu0s} & 2 & - & 1 & $\infty$ & $\infty$ & 0 & 0 & \TT{1g00s} & 2 & 7 & 3 & 24 & 24 & 1 & 1 \\ 
         \TT{fgu0s} & 3 & 5 & 1 & 2058 & 2058 & 190 & 3 & \TT{1g00s} & 3 & 5 & 3 & 4480 & 238544 & 4845 & 37 \\ \hline 
         \TT{fgu00} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{1g000} & 2 & 6 & 4 & 30 & 30 & 1 & 1 \\ 
         \TT{fgu00} & 3 & 5 & 2 & 9686 & 33606 & 1140 & 8 & \TT{1g000} & 3 & 4 & 4 & 668 & 668 & 1 & 1 \\ \hline 
         \TT{fg0vs} & 2 & - & 1 & $\infty$ & $\infty$ & 0 & 0 & \TT{11uvs} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 \\ 
         \TT{fg0vs} & 3 & 5 & 1 & 2058 & 2058 & 190 & 3 & \TT{11uvs} & 3 & 5 & 2 & 57912 & 201265 & 1140 & 8 \\ \hline 
         \TT{fg0v0} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{11uv0} & 2 & 7 & 3 & 48 & 48 & 1 & 1 \\ 
         \TT{fg0v0} & 3 & 5 & 2 & 9686 & 112520 & 1140 & 8 & \TT{11uv0} & 3 & 5 & 3 & 8940 & 477080 & 4845 & 37 \\ \hline 
         \TT{fg00s} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{11u0s} & 2 & 7 & 3 & 36 & 36 & 1 & 1 \\ 
         \TT{fg00s} & 3 & 5 & 2 & 9686 & 33606 & 1140 & 8 & \TT{11u0s} & 3 & 5 & 3 & 8786 & 46192 & 4845 & 37  \\ \hline 
         \TT{fg000} & 2 & 7 & 3 & 18 & 18 & 1 & 1 & \TT{11u00} & 2 & 6 & 4 & 60 & 60 & 1 & 1 \\
         \TT{fg000} & 3 & 5 & 3 & 3884 & 207664 & 4845 & 37 & \TT{11u00} & 3 & 4 & 4 & 1336 & 1336 & 1 & 1 \\ \hline
         \TT{f1uvs} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{110vs} & 2 & 7 & 3 & 72 & 72 &  1 & 1 \\ 
         \TT{f1uvs} & 3 & 5 & 2 & 4111 & 4111 & 190 & 3 & \TT{110vs} & 3 & 5 & 3 & 16390 & 85480 & 4845 & 37  \\ \hline 
         \TT{f1uv0} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{110v0} & 2 & 6 & 4 & 60 & 60 & 1 & 1 \\ 
         \TT{f1uv0} & 3 & 5 & 2 & 29044	& 100816 & 1140 & 8 & \TT{110v0} & 3 & 4 & 4 & 1336 & 1336 & 1 & 1 \\ \hline
         \TT{f1u0s} & 2 & - & 2 & $\infty$ & $\infty$ & 1 & 1 & \TT{1100s} & 2 & 6 & 4 & 60 & 60 & 1 & 1 \\ 
         \TT{f1u0s} & 3 & 5 & 2 & 14760 & 160190 & 1140 & 8 & \TT{1100s} & 3 & 4 & 4 & 1336 & 1336 & 1 & 1 \\ \hline 
         \TT{f1u00} & 2 & 7 & 3 & 18 & 18 & 1 & 1 & \TT{11000} & 2 & 5 & 5 & 20 & 20 & 1 & 1 \\ 
         \TT{f1u00} & 3 & 5 & 3 & 4400 & 244544 & 4845 & 37 & \TT{11000} & 3 & 4 & 5 & 640 & 640 & 1 & 1 \\ \hline
         \TT{f10vs} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{ffuvs} & 2 & - & 1 &$ \infty$ & $\infty$ & 0 & 0\\ 
         \TT{f10vs} & 3 & 5 & 2 & 24332 & 86539 & 1140 & 8 & \TT{ffuvs} & 3 & 5 & 1 & 4617 & 4617 & 190 & 3 \\ \hline 
         \TT{f10v0} & 2 & 7 & 3 & 36 & 36 & 1 & 1 & \TT{ffuv0} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 \\
         \TT{f10v0} & 3 & 5 & 3 & 7764 & 57220 & 4845 & 37 & \TT{ffuv0} & 3 & 5 & 2 & 16188 & 119119 & 1140 & 8 \\ \hline
         \TT{f100s} & 2 & 7 & 3 & 18 & 18 & 1 & 1 & \TT{ffu0s} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 \\
         \TT{f100s} & 3 & 5 & 3 & 4392 & 102778 & 4845 & 37 & \TT{ffu0s} & 3 & 5 & 2 & 29028 & 100758 & 1140 & 8 \\ \hline
         \TT{f1000} & 2 & 6 & 4 & 30 & 30 & 1 & 1 & \TT{ffu00} & 2 & 7 & 3 & 24 & 24 & 1 & 1 \\
         \TT{f1000} & 3 & 4 & 4 & 668 & 668 & 1 & 1 & \TT{ffu00} & 3 & 5 & 3 & 4484 & 176992 & 4845 & 37 \\ \hline
         \TT{1guvs} & 2 & - & 1 & $\infty$ & $\infty$ & 0 & 0 & \TT{ff0vs} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 \\ 
         \TT{1guvs} & 3 & 5 & 1 & 4360 & 4360 & 190 & 3 & \TT{ff0vs} & 3 & 5 & 2 & 38700 & 134352 & 1140 & 8 \\ \hline 
         \TT{1guv0} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 &  \TT{ff0v0} & 2 & 7 & 3 & 24 & 24 & 1 & 1 \\ 
         \TT{1guv0} & 3 & 5 & 2 & 29046 & 100808 & 1140 & 8 & \TT{ff0v0} & 3 & 5 & 3 & 4484 & 92336 & 4845 & 37 \\ \hline 
         \TT{1gu0s} & 2 & - & 2 & $\infty$ & $\infty$ & 0 & 0 & \TT{ff00s} & 2 & 7 & 3 & 36 & 36 & 1 & 1 \\ 
         \TT{1gu0s} & 3 & 5 & 2 & 29024	& 100718 & 1140 & 8 & \TT{ff00s} & 3 & 5 & 3 & 7756 & 396042 & 4845 & 37 \\ \hline 
         \TT{1gu00} & 2 & 7 & 3 & 36 & 36 & 1 & 1 & \TT{ff000} & 2 & 6 & 4 & 30 & 30 & 1 & 1 \\
         \TT{1gu00} & 3 & 5 & 3 & 7760 & 43315 & 4845 & 37 & \TT{ff000} & 3 & 4 & 4 & 668 & 668 & 1 & 1 \\ \hline
    \end{tabular}
    }
\caption{\textbf{80 groups of minimal autocalibration problems} for $M \in \{ 2, 3 \}$ views. For each triplet $(\mathtt{fguvs},M,N)$ we list: \emph{i}) $L$, the number of linear constraints on $K$, \emph{ii}) the minimum and maximum solution count in $\mathbb{C}$, \emph{iii}) $\# \text{subsys.} = \binom{(M-1)\binom{N}{2}}{M+N-L+4}$, the number of square subsystems of~\eqref{eq:depth-equation-2}, \emph{iv}) $\# \bg$, the number of inequivalent minimal relaxations.
The numbers $\# \bg $ and $\textrm{Min } \# \textrm{ sol.}$ are most important, as they measure the number of minimal relaxations and the complexity of solving them. 
Solution counts refer to unknown depths and the parameters of $\omega$ in~\eqref{eq:omega}--\eqref{eq:depth-equation-2}. 
%See SM \cref{SM:Tab:minimal-autocalibration} for solution counts without the parametrization of $\omega$ in~\eqref{eq:omega}.
The two counts $\bullet^\ast$ are only conjectural extrema, due to the prohibitive time needed to check all cases.}
\label{tab:Minimal-Autocalibration-Substitution-Tab}
\vspace{-1.0em}
\end{table*}
